Distributed Learning and Inference with Compressed Images

Modern computer vision requires processing large amounts of data, both while training the model and/or during inference, once the model is deployed. Scenarios where images are captured and processed in physically separated locations are increasingly common (e.g. autonomous vehicles, cloud computing). In addition, many devices suffer from limited resources to store or transmit data (e.g. storage space, channel capacity). In these scenarios, lossy image compression plays a crucial role to effectively increase the number of images collected under such constraints. However, lossy compression entails some undesired degradation of the data that may harm the performance of the downstream analysis task at hand, since important semantic information may be lost in the process. Moreover, we may only have compressed images at training time but are able to use original images at inference time, or vice versa, and in such a case, the downstream model suffers from covariate shift. In this paper, we analyze this phenomenon, with a special focus on vision-based perception for autonomous driving as a paradigmatic scenario. We see that loss of semantic information and covariate shift do indeed exist, resulting in a drop in performance that depends on the compression rate. In order to address the problem, we propose dataset restoration, based on image restoration with generative adversarial networks (GANs). Our method is agnostic to both the particular image compression method and the downstream task; and has the advantage of not adding additional cost to the deployed models, which is particularly important in resource-limited devices. The presented experiments focus on semantic segmentation as a challenging use case, cover a broad range of compression rates and diverse datasets, and show how our method is able to significantly alleviate the negative effects of compression on the downstream visual task.

==> Distributed Learning and Inference Arxiv version/resources.tex <==
\usepackage{float}

\newcommand{\tabletraintestconfigurations}{
	\begin{table}
		\centering
		\caption{Training/test configurations}
		\setlength{\tabcolsep}{1.5pt}
		\begin{tabular}{ccccccc}
				\toprule
				\multirow{2}{*}{Config.} & \multicolumn{2}{c}{Distribution} & \multicolumn{2}{c}{Inf. loss} & \multirow{2}{*}{\begin{tabular}{c}Cov.\\ shift\end{tabular}} & Examples \\
				& Train & Test &  Train & Test & \\
				\midrule
				OO & $p_{X}$ & $p_{X}$ & No & No & No & Most machine learning\\
				CO & $p_{\hat{X}}$ & $p_{X}$ & Yes & No & Large  & \begin{tabular}{c}On-board analysis\\ (autonomous cars, drones)\end{tabular}\\
				OC & $p_{X}$ & $p_{\hat{X}}$ & No & Yes & Large  & \begin{tabular}{c}Cloud computing, \\distributed automotive perception\end{tabular}\\
				CC & $p_{\hat{X}}$ & $p_{\hat{X}}$ &  Yes & Yes & No & \begin{tabular}{c}Compression before \\ training/inference\end{tabular}\\
				\midrule
				OR & $p_{X}$ & $p_{\bar{X}}$ & Yes & No & Medium  & Image restoration\\
				RO & $p_{\bar{X}}$ & $p_{X}$ & No & Yes & Medium  & Dataset restoration\\
				\bottomrule
		\end{tabular}%}
		\label{tab:nomenclature}
	\end{table}
}

\newcommand{\tablemiouperclassfinal}{
\begin{table*}
\centering
\caption{Per class segmentation performance for the configurations OO, CO, RO, AO and CC.}
\setlength{\tabcolsep}{4pt}
\resizebox{\linewidth}{!}{
\begin{tabular}{c|c| ccccccccccccccccccc |cc|c}
\multicolumn{1}{c}{} & \multicolumn{1}{c}{} & & & & & & & & & & & & & & & & & & & \multicolumn{1}{c}{} & \multicolumn{1}{c}{\multirow[c]{8}{*}{\textcolor{blue}{Small}}} & \multicolumn{1}{c}{\multirow[c]{8}{*}{\textcolor{red}{{Big}}}} & \multicolumn{1}{c}{\multirow[c]{8}{*}{\textbf{Mean}}} \\
\multicolumn{1}{c}{} & \multicolumn{1}{c}{\textbf{bpp}} & \rot{\textcolor{red}{Road}} & \rot{\textcolor{red}{Sidewalk}} & \rot{\textcolor{red}{Building}} & \rot{\textcolor{red}{Wall}} & \rot{\textcolor{red}{Fence}} & \rot{\textcolor{red}{Vegetation}} & \rot{\textcolor{red}{Terrain}} & \rot{\textcolor{red}{Sky}} & \rot{\textcolor{red}{Car}} & \rot{\textcolor{red}{Truck}} & \rot{\textcolor{red}{Bus}} & \rot{\textcolor{red}{Train}} & \rot{\textcolor{blue}{Person}} & \rot{\textcolor{blue}{Rider}} & \rot{\textcolor{blue}{Motorcycle}} & \rot{\textcolor{blue}{Bicycle}} & \rot{\textcolor{blue}{Pole}} & \rot{\textcolor{blue}{Traffic light}} & \rot{\textcolor{blue}{Traffic sign}} & \textcolor{blue}{obj.} & \multicolumn{1}{c}{\textbf{\textcolor{red}{obj.}}} & \multicolumn{1}{c}{\textbf{IoU}} \\
\toprule
\parbox[t]{.5mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{CO (MSH)}}} & 0.0419 & 97.27 & 78.29 & 90.13 & 28.36 & 49.32 & 90.31 & 51.83 & 94.33 & 93.91 & 76.13 & 77.56 & 48.08 & 77.94 & 54.00 & 52.55 & 70.39 & 58.80 & 59.20 & 72.95 & 63.69 & 72.96 & 69.55 \\
 & 0.0613 & 97.50 & 79.98 & 91.11 & 32.74 & 50.31 & 91.08 & 57.65 & 93.98 & 94.41 & \textbf{77.82} & 84.76 & 65.35 & \textbf{79.22} & \textbf{57.76} & 61.15 & 73.32 & 59.46 & 62.39 & 73.63 & 66.70 & 76.39 & 72.82 \\
 & 0.0891 & \textbf{97.93} & \textbf{82.79} & 91.44 & 34.13 & 53.66 & 91.40 & 58.81 & 94.63 & 94.72 & 78.28 & 78.73 & 42.79 & \textbf{80.47} & 58.48 & 62.29 & 75.07 & \textbf{62.28} & 64.41 & 76.03 & 68.43 & 74.94 & 72.54 \\
 & 0.1279 & 97.77 & 82.15 & 91.83 & 40.36 & 55.53 & 91.75 & 59.48 & 94.67 & 94.80 & 80.08 & 87.80 & \textbf{75.28} & \textbf{81.16} & 60.36 & 63.99 & 75.34 & 62.49 & 65.16 & 77.20 & 69.39 & 79.29 & 75.64 \\
\midrule[0pt]
\parbox[t]{.5mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{CC (MSH)}}} & 0.0419  & 97.17 & 76.68 & 89.12 & 50.18 & 42.21 & 88.57 & 51.99 & 94.31 & 92.58 & 73.95 & 77.13 & 56.96 & 71.46 & 50.95 & 43.81 & 64.12 & 52.25 & 53.30 & 66.97 & 57.55 & 74.24 & 68.09 \\
& 0.0613  & 97.56 & 79.99 & 90.26 & 51.93 & 46.02 & 89.96 & 59.22 & 94.53 & 93.52 & 77.54 & 81.73 & 52.43 & 74.54 & 54.46 & 52.66 & 68.12 & 55.70 & 56.76 & 70.41 & 61.81 & 76.22 & 70.91 \\
& 0.0891  & 97.70 & 81.17 & 91.03 & 48.93 & 49.88 & 90.82 & 58.53 & 94.83 & 94.18 & 78.69 & 78.60 & 43.80 & 76.86 & 54.80 & 55.03 & 71.61 & 58.81 & 60.41 & 73.77 & 64.47 & 75.68 & 71.55\\
& 0.1279 & \textbf{97.84} & 82.24 & 91.62 & 53.64 & 52.42 & 91.41 & 59.93 & 94.75 & 94.34 & 77.05 & 88.14 & 72.19 & 78.95 & 60.26 & 60.45 & 73.17 & 60.27 & 63.29 & 75.48 & 67.41 & 79.63 & 75.13 \\

\midrule[0pt]
\parbox[t]{.5mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{AO (MSH)}}} & 0.0419 & 97.44 & 79.04 & 90.81 & 44.23 & 47.51 & 90.43 & 56.46 & 94.52 & \textbf{94.32} & \textbf{81.46} & 84.22 & 61.96 & 76.85 & 55.17 & 55.54 & 70.97 & 56.35 & 59.16 & 71.67 & 63.67 & 76.87 & 72.01 \\
& 0.0613 & 97.62 & 80.62 & 91.45 & 51.81 & 51.82 & 91.06 & 57.77 & 94.61 & 94.37 & 76.96 & \textbf{86.44} & \textbf{77.55} & 77.94 & 57.34 & 59.61 & 73.13 & 59.39 & 61.50 & 74.38 & 66.18 & \textbf{79.34} & 74.49 \\
& 0.0891 & 97.57 & 80.62 & 91.83 & 50.42 & 55.02 & 91.53 & 58.70 & 94.90 & 94.77 & 79.81 & 84.40 & 63.53 & 79.35 & 58.43 & \textbf{63.62} & 75.04 & 60.99 & 63.85 & 75.62 & 68.13 & 78.59 & 74.74 \\
& 0.1279 & 97.42 & 80.44 & 92.01 & 52.22 & 55.05 & 91.80 & 59.92 & 94.93 & 95.07 & \textbf{82.16} & 83.85 & 63.37 & 80.23 & 58.78 & 63.35 & 74.88 & 62.23 & 65.63 & 76.60 & 68.82 & 79.02 & 75.26 \\

\midrule[0pt]
\parbox[t]{.5mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{RO (MSH)}}} & 0.0419 & \textbf{97.67} & \textbf{80.85} & \textbf{91.40} & \textbf{51.17} & \textbf{49.80} & \textbf{91.07} & \textbf{59.97} & \textbf{94.87} & 94.30 & 80.74 & \textbf{86.69} & \textbf{70.06} & \textbf{77.95} & \textbf{57.76} & \textbf{61.35} & \textbf{72.64} & \textbf{58.87} & \textbf{61.37} & \textbf{73.47} & \textbf{66.20} & \textbf{79.05} & \textbf{74.32} \\
 & 0.0613 & \textbf{97.97} & \textbf{83.22} & \textbf{91.90} & \textbf{54.29} & \textbf{53.18} & \textbf{91.55} & \textbf{61.23} & \textbf{94.86} & \textbf{94.45} & 76.28 & 82.31 & 68.31 & 78.98 & 57.71 & \textbf{62.51} & \textbf{74.65} & \textbf{60.96} & \textbf{63.92} & \textbf{75.60} & \textbf{67.76} & 79.13 & \textbf{74.94} \\
 & 0.0891 & 97.77 & 82.23 & \textbf{92.28} & \textbf{55.29} & \textbf{57.61} & \textbf{92.04} & \textbf{61.96} & \textbf{94.91} & \textbf{94.99} & \textbf{81.59} & \textbf{86.45} & \textbf{69.66} & 80.28 & \textbf{60.05} & 63.24 & \textbf{75.57} & 61.83 & \textbf{65.48} & \textbf{76.75} & \textbf{69.03} & \textbf{80.57} & \textbf{76.31} \\
 & 0.1279 & 97.77 & \textbf{82.38} & \textbf{92.43} & \textbf{53.87} & \textbf{56.75} & \textbf{92.23} & \textbf{62.40} & \textbf{95.00} & \textbf{95.09} & 79.92 & \textbf{88.71} & 74.90 & 80.84 & \textbf{60.46} & \textbf{66.08} & \textbf{76.59} & \textbf{63.57} & \textbf{67.00} & \textbf{77.61} & \textbf{70.31} & \textbf{80.96} & \textbf{77.03} \\
 
\midrule[1pt]
\parbox[t]{.5mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{CO (BPG)}}} & 0.0454 & 97.49 & 79.67 & 90.34 & 35.84 & 48.22 & 90.73 & 55.80 & 94.03 & 93.87 & 75.86 & 81.80 & 60.63 & 77.44 & 55.50 & 61.08 & 71.01 & 56.55 & 59.69 & 72.75 & 64.86 & 75.36 & 71.49 \\
 & 0.0674 & 97.72 & 81.54 & 91.27 & 41.55 & 51.88 & 91.23 & \textbf{59.61} & 94.77 & 94.36 & 75.77 & 82.64 & 59.23 & 79.19 & 58.28 & 58.26 & 72.98 & 59.39 & 62.70 & 75.16 & 66.56 & 76.80 & 73.03 \\
 & 0.0870 & \textbf{97.98} & \textbf{83.15} & 91.33 & 44.33 & 52.73 & 91.42 & 58.81 & \textbf{94.90} & 94.46 & 75.11 & 81.91 & 58.77 & 79.82 & 58.48 & 62.55 & 74.21 & 59.75 & 62.04 & 75.46 & 67.47 & 77.08 & 73.54 \\
 & 0.1279 & \textbf{97.87} &\textbf{83.10} & 92.06 & 51.82 & 56.04 & 91.94 & 60.49 & \textbf{95.11} & 94.62 & 80.75 & 87.25 & \textbf{75.90} & 80.60 & 60.60 & 63.86 & 74.68 & 62.29 & 65.56 & 76.95 & 69.22 & \textbf{80.58} & \textbf{76.39} \\
\midrule[0pt]
\parbox[t]{.5mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{CC (BPG)}}} & 0.0454  & 97.03 & 76.14 & 88.66 & 41.33 & 42.06 & 88.48 & 53.96 & 94.08 & 92.54 & 72.33 & 76.42 & 55.60 & 70.82 & 50.47 & 48.80 & 63.93 & 51.06 & 53.41 & 66.92 & 57.92 & 73.22 & 67.58 \\
& 0.0674  & 97.46 & 79.06 & 90.15 & 47.74 & 47.00 & 89.68 & 57.99 & 94.42 & 93.27 & 72.14 & 79.84 & 59.16 & 74.33 & 53.64 & 48.00 & 67.46 & 55.30 & 57.01 & 70.92 & 60.95 & 75.66 & 70.24 \\
& 0.0870  & 97.58 & 80.22 & 90.50 & 47.41 & 47.20 & 90.25 & 58.40 & 94.54 & 93.58 & 75.20 & 83.35 & 57.80 & 75.77 & 54.76 & 52.58 & 69.71 & 56.64 & 57.73 & 72.09 & 62.75 & 76.34 & 71.33 \\
& 0.1279 & 97.71 & 81.28 & 91.35 & 49.49 & 52.74 & 91.10 & 58.25 & 94.82 & 94.16 & 73.89 & \textbf{88.41} & 70.80 & 78.11 & 58.23 & 58.27 & 72.40 & 59.67 & 61.75 & 74.68 & 66.16 & 78.67 & 74.06 \\

\midrule[0pt]
\parbox[t]{.5mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{AO (BPG)}}} & 0.0454 & 97.51 & 79.73 & 91.04 & 45.38 & 48.27 & 90.81 & \textbf{57.10} & 94.55 & \textbf{94.36} & \textbf{81.44} & 85.13 & \textbf{74.56} & 77.34 & 56.23 & 58.89 & 72.52 & 57.51 & 61.33 & 72.30 & 65.16 & 78.25 & 73.47 \\
& 0.0674 & 97.67 & 81.13 & \textbf{91.86} & \textbf{54.33} & 54.61 & 91.40 & 57.30 & 94.82 & 94.46 & \textbf{82.53} & 84.56 & 63.39 & 78.86 & \textbf{57.97} & 58.46 & 73.55 & 60.17 & 63.75 & 74.09 & 66.69 & 78.99 & 74.47\\
& 0.0870 & 97.42 & 80.18 & 91.89 & 53.25 & 51.30 & 91.65 & \textbf{59.39} & 94.65 & 94.64 & 78.62 & 85.76 & 69.54 & 79.71 & 59.47 & 59.62 & \textbf{74.63} & 61.01 & 63.92 & 75.82 & 67.74 & 79.02 & 74.87\\
& 0.1279 & 97.70 & 81.86 & 92.04 & 48.35 & 52.93 & 91.94 & \textbf{62.68} & 95.03 & 94.91 & \textbf{81.08} & 88.30 & 71.81 & 80.72 & \textbf{60.90} & \textbf{64.78} & 75.66 & 62.09 & 65.61 & 77.13 & 69.56 & 79.89 & 76.08 \\

\midrule[0pt]
\parbox[t]{.5mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{RO (BPG)}}} & 0.0454 & \textbf{97.78} & \textbf{81.69} & \textbf{91.52} & \textbf{50.05} & \textbf{52.45} & \textbf{91.24} & 56.78 & \textbf{94.97} & 94.18 & 78.88 & \textbf{86.13} & 73.22 & \textbf{77.88} & \textbf{56.31} & \textbf{62.19} & \textbf{73.15} & \textbf{59.39} & \textbf{62.81} & \textbf{74.47} & \textbf{66.60} & \textbf{79.07} & \textbf{74.48} \\
 & 0.0674 & \textbf{97.95} & \textbf{82.89} & 91.84 & 48.17 & \textbf{52.14} & \textbf{91.57} & 59.47 & \textbf{94.85} & \textbf{94.53} & 78.86 & \textbf{85.97} & \textbf{76.59} & \textbf{79.37} & \textbf{58.51} & \textbf{62.00} & \textbf{74.07} & \textbf{60.90} & \textbf{65.14} & \textbf{75.25} & \textbf{67.89} & \textbf{79.57} & \textbf{75.27} \\
 & 0.0870 & 97.71 & 81.73 & \textbf{92.13} & \textbf{52.62} & \textbf{54.76} & \textbf{91.75} & 56.93 & 94.82 & \textbf{94.81} & \textbf{83.52} & \textbf{88.36} & \textbf{78.94} & \textbf{80.10} & 59.45 & \textbf{62.72} & \textbf{74.63} & \textbf{62.07} & \textbf{64.93} &\textbf{76.44} & \textbf{68.62} & \textbf{80.67} & \textbf{76.23} \\
 & 0.1279 & 97.58 & 81.57 & \textbf{92.54} & \textbf{53.23} &\textbf{58.71} & \textbf{92.05} & 61.16 & 94.85 & \textbf{95.05} & 79.79 & 85.14 & 69.27 & \textbf{80.91} & 60.34 & \textbf{64.78} & \textbf{76.11} & \textbf{63.11} & \textbf{66.83} & \textbf{77.84} & \textbf{69.99} & 80.08 & 76.36 \\
\midrule[1pt]
{\setlength{\tabcolsep}{0pt} \begin{tabular}{c}{OO}\\(PNG)\end{tabular}} & 9.02 & 98.17 & 85.04 & 92.84 & 54.96 & 61.15 & 92.63 & 64.62 & 95.05 & 95.50 & 85.62 & 87.02 & 70.18 & 82.57 & 63.08 & 66.79 & 78.00 & 64.95 & 69.70 & 78.69 & 71.97 & 81.90 & 78.24 \\
\bottomrule
\end{tabular}}
\label{tab:cityscapes-per_class_miou}
\end{table*}
}

\newcommand{\tablehybridtrainingsets}{
\begin{table}
\centering
\caption{Segmentation performance of hybrid training sets compared against other configurations.}
\begin{tabular}{cccccccc}
\toprule
Compression method & CO & rO & o+c O & o+r O  \\ \midrule[1pt]
MSH at 0.0419 bpp & 69.55 & 74.07 & \textbf{75.96} & 73.99 \\
MSH at 0.0891 bpp & 72.54 & 75.69 & \textbf{77.08} & 75.88 \\
\midrule[0pt]
BPG at 0.0454 bpp & 71.49 & 72.32 & \textbf{74.42} & 73.98 \\
BPG at 0.0674 bpp & 73.03 & 74.01 & 75.87 & \textbf{76.12} \\
BPG at 0.0870 bpp & 73.54 & 75.15 & 75.98 &\textbf{76.67} \\
\bottomrule
\end{tabular}
\label{tab:hybridtrainingsets}

\vspace{0.5em} The original images form 12.5\% of all mixtures and the configuration oO results in a performance of 71.90. The IoU of the \textit{Train} class affects the mIoU dramatically affects BPG at 0.0454 bpp. When \textit{Train} class is excluded from mIoU, the values for o+c O and o+r O become 74.59 and \textbf{74.96}.

\end{table}
}

\newcommand{\tableperceptualindices}{
\begin{table}
\centering
\caption{Perceptual indices of different image sets.}
\resizebox{\linewidth}{!}{
\begin{tabular}{cccccc}
\toprule
& & &  
\multicolumn{3}{c}{Restoration type} \\
\multirow{2}{*}{\centering Compression method}& \multirow{2}{*}{Original}  & \multirow{2}{*}{Compressed} & \multirow{2}{*}{Adversarial} & \multicolumn{2}{c}{Non Adversarial} \\
& & & & RDN - P & RDN - M  \\
\midrule
MSH at 0.0419 bpp & 40.21 & 55.69 & 40.56 &  55.40 &  55.82\\
\midrule
BPG at 0.0674 bpp & 40.21 & 52.95 & 41.10 &  53.69 &  53.62 \\
\bottomrule
\end{tabular}}
\label{tab:perceptualindices}

\vspace{0.5em} RDN - P and RDN - M stand for RDN (PSNR) and RDN (MS-SSIM) respectively. The perceptual indices are calculated using the Blind image quality assessment method of HOSA~\cite{xu2016blind}.

\end{table}
}

\newcommand{\tablenewrdnresults}{
\begin{table}
\centering
\caption{Comparison of adversarial restoration against RDN in various metrics.}
\setlength{\tabcolsep}{4pt}
\resizebox{\columnwidth}{!}{
\begin{tabular}{cccccc}
\toprule
\multirow{3}{5em}{\centering Compression method} & \multirow{3}{5em}{\centering Evaluation metric} &  \multicolumn{4}{c}{\centering Restoration type}\\
&  & None & \multicolumn{2}{c}{Non adversarial} & Adversarial \\
& & (CO) & RDN - P & RDN - M & (RO) \\
\midrule[1pt]
\multirow{3}{5em}{ \centering MSH at 0.0419 bpp } & mIoU & 69.55 & 71.63 & 71.82 & \textbf{74.32} \\
&PSNR (dB) & 33.47 & \textbf{33.67} & 33.51 & 31.55 \\
&MS-SSIM (dB) & 13.43 & \textbf{13.66}& \textbf{13.66} & 11.87 \\
\midrule[0pt]

\multirow{3}{5em}{\centering MSH at 0.0613 bpp } & mIoU & 72.82 & 72.39 & 71.92 & \textbf{74.94} \\
&PSNR (dB) & 35.00 & \textbf{35.17} & 35.00 & 32.86 \\
&MS-SSIM (dB) & 14.90 & \textbf{15.11} & \textbf{15.10} & 13.08 \\
\midrule[0pt]

\multirow{3}{5em}{\centering BPG at 0.0454 bpp } & mIoU & 71.49 & 70.91 & 69.58 & \textbf{74.48} \\
&PSNR (dB) & 33.37 & \textbf{34.04} & 33.62 & 31.95  \\
&MS-SSIM (dB) & 12.96 & \textbf{13.58}  & \textbf{13.57} & 11.74 \\
\midrule[0pt]

\multirow{3}{5em}{\centering BPG at 0.0674 bpp } & mIoU & 73.03 & 73.26 & 73.96 & \textbf{75.27} \\
& PSNR (dB) & 34.81 & \textbf{35.56} & 35.19 & 33.40 \\
& MS-SSIM (dB) & 14.31 & \textbf{14.99} & \textbf{14.96} & 13.01 \\
\bottomrule
\end{tabular}
}

\vspace{0.5em} RDN - P and RDN - M stand for RDN (PSNR) and RDN (MS-SSIM).

\label{tab:rdn_results}
\end{table}
}


\newcommand{\tableefficiency}{
\begin{table}
\centering
\caption{Inference times for different approaches.}
\begin{tabular}{c cc}
\toprule
\multirow{2}{5em}{\centering Compression method} & Segment & Encode + Decode + Segment  \\
& OO / CO / RO & CC \\
\midrule
MSH & 0.64s & 0.10s + 0.13s + 0.64s = 0.87s \\
BPG & 0.64s & 1.10s + 0.15s + 0.64s = 1.89s \\
\bottomrule
\end{tabular}
\label{tab:efficiency}

\vspace{0.5em} Note that Encode and Decode times for MSH and BPG are measured on a GPU and a CPU respectively. Segmentation time is measured on a GPU. 
\end{table}
}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\figuredatacollection}{

\setlength{\fboxsep}{0pt}
\begin{figure*}[htbp]
	\centering
	{\setlength{\tabcolsep}{3pt}
	 \renewcommand{\arraystretch}{1.5}
	\begin{tabular}{ccc}
		\includegraphics[width=0.4\textwidth]{Pictures/AD_data_collection.pdf} & {\setlength{\tabcolsep}{0pt}
			\renewcommand{\arraystretch}{0}
			\raisebox{\height}{\begin{tabular}{ccc}
			\includegraphics[width=0.1\textwidth]{Pictures/crops/crop1_ground_truth.png} & \includegraphics[width=0.1\textwidth]{Pictures/crops/crop1_input.png} & \includegraphics[width=0.1\textwidth]{Pictures/crops/crop1_reconstructed.png}\\
			\fcolorbox{red}{white}{\includegraphics[width=0.1\textwidth]{Pictures/crops/crop2_ground_truth.png}} & \fcolorbox{red}{white}{\includegraphics[width=0.1\textwidth]{Pictures/crops/crop2_input.png}} & \fcolorbox{red}{white}{\includegraphics[width=0.1\textwidth]{Pictures/crops/crop2_reconstructed.png}}\\
			\fcolorbox{green}{white}{\includegraphics[width=0.1\textwidth]{Pictures/crops/crop3_ground_truth.png}} & \fcolorbox{green}{white}{\includegraphics[width=0.1\textwidth]{Pictures/crops/crop3_input.png}} & \fcolorbox{green}{white}{\includegraphics[width=0.1\textwidth]{Pictures/crops/crop3_reconstructed.png}}\\			 \parbox{0.1\textwidth}{\centering\small Captured} & \parbox{0.1\textwidth}{\centering\small Compressed} & \parbox{0.1\textwidth}{\centering\small Restored}
		\end{tabular}} } & 
		\raisebox{0.\height}{\includegraphics[width=0.15\textwidth]{Pictures/intro_miou.pdf}} \\
		(a) & (b) & (c)
	\end{tabular}
}
	\caption{Problem statement and proposed approach: (a) data collection using lossy compression makes training (top) and test data (bottom) different, (b) differences between test and training data are alleviated using adversarial restoration, and (c) drop in segmentation performance due to lossy compressed training data (CO/CC) and benefit from the proposed restoration method (RO).}
	\label{fig:feature_vis}
\end{figure*}
}

\newcommand{\figuredegradationexamples}{
	\begin{figure*}
		\centering
		\includegraphics[width=\textwidth]{Pictures/crops/section3_crop_c1_edited.png}
		\includegraphics[width=\textwidth]{Pictures/crops/section3_crop_c2_edited.png}
		\includegraphics[width=\textwidth]{Pictures/crops/section3_crop_c3_edited.png}
		\caption{Effects of compression and restoration (from left to right): captured image, compressed (BPG), restored (BPG), compressed (MSH), restored (MSH). The brightness of the image crops have been slightly enhanced to improve visibility.}
		\label{fig:degradationexamples}
	\end{figure*}
}

\newcommand{\figuremcc}{
	\begin{figure}
		\centering
		\includegraphics[width=0.99\columnwidth]{Pictures/mcc.pdf}
		\caption{Example of OC configuration: mobile cloud computing with inference on compressed test images, and high quality training images.}
			\label{fig:mcc}
\end{figure}}

\newcommand{\figureaadaptationmethods}{
    \begin{figure}
		\centering
		{
	        \includegraphics[width=0.99\columnwidth]{Pictures/compressionbeforetraining.pdf}\\
			(a)\\
	        \includegraphics[width=0.99\columnwidth]{Pictures/compressionbeforeinference.pdf}\\
			(b)\\
	        \includegraphics[width=0.99\columnwidth]{Pictures/datasetrestoration.pdf}\\
	        (c)
		}
	\caption{Adaptation strategies: (a) compression before training, (b) compression before inference, and (c) dataset restoration.}
	\label{fig:adaptation_methods}
	\end{figure}
}

\newcommand{\figureilluspercepdist}{
\begin{figure}
    \centering
    \includegraphics[width=.73\columnwidth]{Pictures/percep-dist.pdf}
    \caption{Illustration of the perception-distortion tradeoff~\cite{blau2018perception,blau2019rethinking}. Restoration process shifts the compressed images from a point of low distortion and low perceptual quality to a point of higher distortion but higher perceptual quality in the perception-distortion plane.}
    \label{fig:illus_percep_dist}
\end{figure}
}

\newcommand{\figurecityscapesrdcurvesnew}{
\begin{figure}
    \centering
    \includegraphics[width=0.99\columnwidth]{Pictures/cityscapes_rd_curves.png}
    \caption{Rate-distortion curves for Cityscapes for BPG and MSH, and with and without adversarial image restoration.}
    \label{fig:cityscapes_rd_curves}
\end{figure}
}

\newcommand{\figurecityscapessegmentationperformance}{
\begin{figure}
    \centering
    \includegraphics[width=0.99\columnwidth]{Pictures/cityscapes_exponential_segmentation.pdf}
    \caption{Segmentation performance on Cityscapes for different training/test configurations. }
    \label{fig:cityscapes-segmentation-performance}
\end{figure}
}

\newcommand{\figurerestorationdatarequirednew}{
\begin{figure}
    \centering
    \includegraphics[width=0.99\columnwidth]{Pictures/restoration_data_required_v3.png}
    \caption{Performance of models with different configurations obtained by varying the amount of privileged data.}
    \label{fig:restoration_data-required}
\end{figure}
}

\newcommand{\figurecostperformance}{
	\begin{figure*}
		\centering
		\includegraphics[width=0.99\textwidth]{Pictures/cost_performance.png}
		\caption{Segmentation performance of each configuration against cost of collecting data. Marker size indicates rate.}
		\label{fig:costperformance}
	\end{figure*}
}

\newcommand{\figureadversarialvsnonadversarial}{
	\begin{figure}
		\centering
		\includegraphics[width=0.99\columnwidth]{Pictures/msh_bpg.png}\\
	\caption{Adversarial dataset restoration vs non-adversarial: While Table~\ref{tab:perceptualindices} describes the average perceptual index of the original, compressed and restored image sets, this figure shows the distribution of the perceptual index. Dataset restoration with adversarial image restoration can recover the distribution of the perceptual indices of the original images, while non-adversarial cannot.}
		\label{fig:adversarial_vs_nonadversarial}
	\end{figure}
}

\newcommand{\figureimagesfeatcorr}{
\begin{figure}
    \centering
    \includegraphics[width=0.96\columnwidth]{Pictures/feat_corr.pdf}
    \caption{Feature correlation between segmentation features (at a shallow layer) of the segmentation model trained on raw images. Dataset restoration with adversarial image restoration can recover the distribution of perceptual index and segmentation features of the optimal case (OO), while non-adversarial cannot.}
    \label{fig:images_feat_corr}
\end{figure}
}

\newcommand{\figureaidsegmentationperformance}{
\begin{figure}
    \centering
    \includegraphics[width=0.99\columnwidth]{Pictures/aid_exponential_segmentation.pdf}
    \caption{Segmentation performance on INRIA Aerial Images Dataset for different training/test configurations.}
    \label{fig:aid-segmentation-performance}
\end{figure}
}

\newcommand{\figureaidexample}{
	\begin{figure*}
		\centering
		\includegraphics[width=0.75\textwidth]{Pictures/aid_crop.png}
		\includegraphics[width=0.50\textwidth]{Pictures/aid_seg_crop.png}
		\caption{Top: (from left to right) - captured image, compressed (BPG), restored (BPG), compressed (MSH), restored (MSH). Bottom: Prediction map and accuracy score of segmentation models with different configurations.}
		\label{fig:aidexample}
	\end{figure*}
}



\newcommand{\figuresddsegmentationperformance}{
\begin{figure}
    \centering
    \includegraphics[width=0.99\columnwidth]{Pictures/sdd_exponential_segmentation.pdf}
    \caption{Segmentation performance on Semantic Drones Dataset for different training/test configurations.}
    \label{fig:sdd-segmentation-performance}
\end{figure}
}

\newcommand{\figuremsharch}{
\begin{figure}
    \centering
    \includegraphics[width=0.98\columnwidth]{Pictures/MSH_architecture.pdf}
    \caption{MSH Architecture: Refer to \cite{minnen2018joint} for details on Fully Factorized Entropy Model and Range Encoder-Decoder.}
    \label{fig:msh_arch}
\end{figure}
}


